A Game-Theoretic Framework for Joint Forecasting and Planning

Planning safe robot motions in the presence of humans requires reliable forecasts of future human motion. However, simply predicting the most likely motion from prior interactions does not guarantee safety. Such forecasts fail to model the long tail of possible events, which are rarely observed in limited datasets. On the other hand, planning for worst-case motions leads to overtly conservative behavior and a "frozen robot". Instead, we aim to learn forecasts that predict counterfactuals that humans guard against. We propose a novel game-theoretic framework for joint planning and forecasting with the payoff being the performance of the planner against the demonstrator, and present practical algorithms to train models in an end-to-end fashion. We demonstrate that our proposed algorithm results in safer plans in a crowd navigation simulator and real-world datasets of pedestrian motion. We release our code at https://github.com/portal-cornell/Game-Theoretic-Forecasting-Planning.

==> inputs/evaluation.tex <==
\section{Evaluation}

% \subsection{Baselines}
% MLE forecasting
% Behavior cloning
% [Other approaches that folks try on Crowdnav Kushal Kedia?)

\subsection{Metrics}
% How quickly did everyone reach the goal? How smooth was the motion? Collision?

We consider the following metrics for off-policy evaluation:
\begin{itemize}
    \item \textbf{Average Displacement Error (ADE)}: We measure the distance between the predicted plan and the ground truth plan and average it over all the timesteps in the planning horizon.
    \item \textbf{Final Displacement Error (ADE)}: We measure the distance between the predicted robot plan and the ground truth plan at the end of the planning horizon.
    \item \textbf{Collision Rate}: We measure the percentage of test cases where the predicted robot plans is within collision radius of the humans in the scene.
    
\end{itemize}

\subsection{CrowdNav}

CrowdNav \cite{chen2019crowd} is an open-source multi-agent simulator. It contains a robot and five humans following dynamics. \citeauthor{chen2019crowd} \cite{chen2019crowd} train a reinforcement learning (RL) agent on the simulator that models the interactions between robots and humans using a self-attention mechanism. We collect a dataset of 5000 trajectories using the pre-trained RL agent for our experiments.

We define the following cost function for our experiments:

$C({\xi}_R, {\hat\xi}_H) = \sum_{s_r, s_h \sim {\xi}_R, {\hat\xi}_H)} CHOMP-col-cost (s_r, s_h)$

\subsubsection{On-Policy Evaluation}
We consider the following metrics for off-policy evaluation.
\begin{itemize}
    \item \textbf{Success Rate}: Percentage of episodes where the robot reaches its goal location before timeout.
    \item \textbf{Collision Rate}: Percentage of episodes where the robot comes within the collision radius of one of the humans in the scene.
\end{itemize}

\subsubsection{Off-Policy Evaluation}
In this section, we measure the evaluate the predicted robot plan on the following metrics:


\input{inputs/tables/crowdnav_offpolicy.tex}

\subsubsection{On-Policy Evaluation}

\input{inputs/tables/crowdnav_onpolicy.tex}
% Demonstrations coming from ORCA

% Use a discrete library of trajectories 

% Show that unlike MLE, this guards better against simulated rare events

%Show that unlike BC, this does not just cut off 

\subsubsection{Results}

\begin{itemize}
    \item H1: Forecasting approaches Class B/C should do at least as good as Planner only approach (Class A)
    \item H2: Class C (and Class B with collision loss) should do better at avoiding collisions as it trained for the outcome
    \item H3 [On-policy]: Class C should outperform B or A in rare hazardous situations
    
\end{itemize}

\subsection{Real-World Datasets}
% Use ETH datasets for real world pedestrian data https://arxiv.org/pdf/2001.03093.pdf

% Train an MLE forecaster on this data

% Pick out datapoints where the forecaster is unable to predict anomalous behavior

% On those datapoints, run the robot closed loop, that is use the forecaster to plan paths and execute those paths. Other humans move as they do in the data. Show that you collide as a result (You can limit the episode length of this sim to minimize shift between off and onpolicy)

%Now run with your forecaster and show better guarding


==> inputs/tables/comments.tex <==

% \begin{table*}
% \centering
% \caption{Table comparing the costs of the MLE-Forecaster, ADV-Forecaster when calculated with different planners}
% \label{tab:costs_forecasts}
% \begin{tblr}{
%   row{1} = {c},
%   row{2} = {c},
%   row{6} = {c},
%   cell{1}{1} = {r=2}{},
%   cell{1}{2} = {c=3}{},
%   cell{1}{5} = {c=3}{},
%   cell{1}{8} = {c=3}{},
%   cell{3}{1} = {c},
%   cell{3}{2} = {c},
%   cell{3}{3} = {c},
%   cell{3}{4} = {c},
%   cell{3}{5} = {c},
%   cell{4}{1} = {c},
%   cell{4}{2} = {c},
%   cell{4}{3} = {c},
%   cell{4}{4} = {c},
%   cell{4}{5} = {c},
%   cell{5}{1} = {c},
%   cell{5}{2} = {c},
%   cell{5}{3} = {c},
%   cell{5}{4} = {c},
%   cell{5}{5} = {c},
%   cell{7}{1} = {c},
%   cell{7}{2} = {c},
%   cell{7}{3} = {c},
%   cell{7}{4} = {c},
%   cell{7}{5} = {c},
%   cell{8}{1} = {c},
%   cell{8}{2} = {c},
%   cell{8}{3} = {c},
%   cell{8}{4} = {c},
%   cell{8}{5} = {c},
%   cell{9}{2} = {c},
%   cell{9}{4} = {c},
%   cell{9}{5} = {c},
%   cell{9}{6} = {c},
%   cell{9}{8} = {c},
%   cell{9}{9} = {c},
%   cell{9}{10} = {c},
%   vline{1-3,6,9} = {1}{},
%   vline{5,8,11} = {2}{},
%   vline{1-2,5,8,11} = {3-9}{},
%   hline{1,3,9-10} = {-}{},
%   hline{2} = {2-10}{},
% }
% Datasets         & MLE-Forecaster         &                        &                  & Adv-Forecaster        &                        &                  & Observed Futures      &                        &                  \\
%                  & {Nom-\\Planner\\ Cost} & {Safe-\\Planner\\Cost} & {Observed\\Cost} & {Nom-\\Planner\\Cost} & {Safe-\\Planner\\Cost} & {Observed\\Cost} & {Nom-\\Planner\\Cost} & {Safe-\\Planner\\Cost} & {Observed\\Cost} \\
% \textit{ETH UCY} &                        &                        &                  &                       &                        &                  &                       &                        &                  \\
% ETH              &                        &                        &                  &                       &                        &                  &                       &                        &                  \\
% Hotel            &                        &                        &                  &                       &                        &                  &                       &                        &                  \\
% Univ             & 0.012                  &                        & 0.013            & 0.019                 & 0.011                  & 0.024            & 0.013                 & 0.018                  & 0                \\
% Zara-1           &                        &                        &                  &                       &                        &                  &                       &                        &                  \\
% Zara-2           &                        &                        &                  &                       &                        &                  &                       &                        &                  \\
% Crowd-Nav        & 1.28\%                 &                        & 1.10\%           & 1.11\%                & 0.94\%                 &                  & 1.02\%                & 0.82\%                 & 0                
% \end{tblr}
% \end{table*}

% \begin{table*} [t!]
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lccccc}
% \toprule
% & {Fuel Consumption} & {Instability} & {Stray} & {Subdominance} & {True Reward} \\
% \midrule
% {\textsc{OWLS}}     & {0.179 \small{$\pm$ 0.002}} & {\textbf{0.005} \small{$\pm$ 0.001}} & {\textbf{0.117} \small{$\pm$ 0.005}} & {\textbf{0.074} \small{$\pm$ 0.008}} & {108.470 \small{$\pm$ 2.788}} \\
% {\textsc{BC-top}}   & {\textbf{0.168} \small{$\pm$ 0.029}} & {0.009 \small{$\pm$ 0.002}} & {0.127 \small{$\pm$ 0.012}} & {0.076 \small{$\pm$ 0.043}} & {\textbf{116.490} \small{$\pm$ 5.119}}  \\
% {\textsc{BC-all}}   & {0.186 \small{$\pm$ 0.012}} & {0.010 \small{$\pm$ 0.002}} & {0.128 \small{$\pm$ 0.004}} & {0.097 \small{$\pm$ 0.018}} & {95.686 \small{$\pm$ 4.858}}  \\
% \midrule
% {\textsc{IQL (true reward)}}& {0.193 \small{$\pm$ 0.005}} & {\textbf{0.005} \small{$\pm$ 0.001}} & {0.154 \small{$\pm$ 0.006}} & {0.123 \small{$\pm$ 0.012}} & {95.147 \small{$\pm$ 4.185}} \\
% {\textsc{BC-top (training data)}}  & 0.094 \small{$\pm$ 0.009} & 0.0 \small{$\pm$ 0.0} & 0.038 \small{$\pm$ 0.016} & --- & 207.384 \small{$\pm$ 5.527}\\
% {\textsc{BC-all (training data)}} & 0.165 \small{$\pm$ 0.073} & 0.0 \small{$\pm$ 0.009} & 0.062 \small{$\pm$ 0.037}  & --- & 142.501 \small{$\pm$ 48.638} \\
% \bottomrule
% \end{tabular}}
% \caption{Subcost results of our algorithm against various baselines, where lower cost is better. For each agent, we train 5 checkpoints and evaluate each on 200 rollouts per checkpoint. We normalize each subcost between [0,1], and report the mean and standard deviation of subcosts across the 5 checkpoints. We also report the total subdominance between test trajectories and training trajectories, as well as the true reward as given by the environment.}
% \label{tbl:subdom-results}
% \end{table*}


==> inputs/tables/costs_forecaster.tex <==
\begin{table*}
\centering
\captionsetup{justification=centering}
\caption{We compare the costs (Eq. \ref{eq:chomp_cost}) of different combinations of planners and forecasters (including the observed future motions of the agents) on the testing splits of the \textsc{ETH-UCY} benchmark and the \textsc{CrowdNav} simulator. For each forecaster, we mark in bold the planner with lower cost.}
\label{tab:costs_forecasts}
\resizebox{\textwidth}{!}{
\begin{tblr}{
  % width = \linewidth,
  % colspec = {Q[62]Q[100]Q[85]Q[88]Q[25]Q[100]Q[98]Q[75]Q[25]Q[100]Q[98]Q[75]},
  column{even} = {c},
  column{3} = {c},
  column{7} = {c},
  column{11} = {c},
  cell{1}{1} = {r=2}{},
  cell{1}{2} = {c=3}{0.273\linewidth},
  cell{1}{6} = {c=3}{0.273\linewidth},
  cell{1}{10} = {c=3}{0.273\linewidth},
  cell{3}{1} = {c},
  cell{4}{1} = {c},
  cell{5}{1} = {c},
  cell{6}{1} = {c},
  cell{7}{1} = {c},
  cell{8}{1} = {c},
  cell{9}{1} = {c},
  hline{1,10} = {-}{0.15em},
  hline{2} = {2-4,6-8, 10-12}{0.05em},
  hline{3} = {-}{0.10em},
  % hline{8} = {-}{0.05em},
  hline{8} = {-}{0.10em},
  % fontsize = {7cm},
  % hline{9} = {2-12}{},
}
& \textsc{MLE-Forecaster} &              &             &  & \textsc{Adv-Forecaster} &              &             &  & \textsc{Observed Futures} &              &             \\
            & \textsc{Nom-Planner}    & \textsc{Safe-Planner} & \textsc{Obs. Plan} &  & \textsc{Nom-Planner}    & \textsc{Safe-Planner} & \textsc{Obs. Plan} &  & \textsc{Nom-Planner}    & \textsc{Safe-Planner} & \textsc{Obs. Plan} \\
\textsc{Univ}        & \textbf{0.024}          & 0.025        & 0.020        &  & \textbf{0.025}          & \textbf{0.025}        & 0.021       &  & \textbf{0.020}             & \textbf{0.020}         & 0           \\
\textsc{ETH}         & \textbf{0.003}          & \textbf{0.003}        & 0.008       &  & \textbf{0.002}          & \textbf{0.002}        & 0.004       &  & \textbf{0.008}            & 0.010         & 0           \\
\textsc{Hotel}       & \textbf{0.006}          & 0.007        & 0.008       &  & 0.008          & \textbf{0.007}        & 0.009       &  & 0.008            & \textbf{0.007}        & 0           \\
\textsc{Zara1}       & \textbf{0.004}          & 0.005        & 0.005       &  & \textbf{0.005}          & \textbf{0.005}        & 0.005       &  & \textbf{0.005}            & 0.006        & 0           \\
\textsc{Zara2}       & \textbf{0.009}          & 0.011        & 0.008       &  & \textbf{0.010}           & \textbf{0.010}         & 0.008       &  & \textbf{0.008}            & 0.009        & 0           \\
\textbf{\textsc{ETH-UCY}} (Avg.) & \textbf{0.009}         & 0.010       & 0.010      &  & \textbf{0.010}           & \textbf{0.010}       & 0.009      &  & \textbf{0.010}           & \textbf{0.010}       & 0           \\
\textbf{\textsc{Crowd-Nav}}   & 0.019          & \bf 0.014        & 0.007       &  & 0.055          & \bf 0.029        & 0.043       &  & 0.017            & \textbf{0.011}        & 0           
\end{tblr}
}
\end{table*}

==> inputs/tables/costs_planner.tex <==
\begin{table*}[ht!]
\caption{Table comparing the costs of the MLE-Planner and Safe-Planner \\ with the Ground Truth futures, MLE-Forecaster and the Adv-Forecaster}
\captionsetup{justification=centering}
\centering
\label{tab:costs_planner}
\begin{tabular}{|c|ccc|cll|}
\hline
\multirow{2}{*}{Datasets}       & \multicolumn{3}{c|}{MLE-Planner}                                                                                                                                                                             & \multicolumn{3}{c|}{Safe-Planner}                                                                                                                                                                                                                     \\ \cline{2-7} 
                                & \begin{tabular}[c]{@{}c@{}}Cost with\\ Ground Truth\end{tabular} & \begin{tabular}[c]{@{}c@{}}Cost with \\ MLE-Forecaster\end{tabular} & \begin{tabular}[c]{@{}c@{}}Cost with \\ ADV-Forecaster\end{tabular} & \begin{tabular}[c]{@{}c@{}}Cost with\\ Ground Truth\end{tabular} & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Cost with \\ MLE-Forecaster\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Cost with \\ ADV-Forecaster\end{tabular}} \\ \hline
\textit{ETH \& UCY}             &                                                                  &                                                                     &                                                                     &                                                                  &                                                                                         &                                                                                          \\
ETH                             &                                                                  &                                                                     &                                                                     &                                                                  &                                                                                         &                                                                                          \\
Hotel                           &                                                                  &                                                                     &                                                                     &                                                                  &                                                                                         &                                                                                          \\
Univ                            &                                                                  &                                                                     &                                                                     &                                                                  &                                                                                         &                                                                                          \\
Zara-1                          &                                                                  &                                                                     &                                                                     &                                                                  &                                                                                         &                                                                                          \\
Zara-2                          &                                                                  &                                                                     &                                                                     &                                                                  &                                                                                         &                                                                                          \\ \hline
\multicolumn{1}{|l|}{Crowd-Nav} & \multicolumn{1}{l}{}                                             & \multicolumn{1}{l}{}                                                & \multicolumn{1}{l|}{}                                               & \multicolumn{1}{l}{}                                             &                                                                                         &                                                                                          \\ \hline
\end{tabular}
\end{table*}

==> inputs/tables/crowdnav_offpolicy.tex <==
\begin{table}
\label{tab:crowdnav_off}
\caption{Off-Policy Evaluation on CrowdNav environment}
\centering
\begin{tabular}{l|l|l|l|l|l}
\textbf{Method}                                                                                     & \textbf{ADE} & \textbf{FDE} & \begin{tabular}[c]{@{}l@{}}\textbf{One-}\\\textbf{Step }\\\textbf{Error}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Col. Rate}\\\textbf{(0.6 dist)}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{\textbf{Col. Rate}}\\\textbf{\textbf{(0.4 dist)}}\end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Vanilla IL \\(Class A)\end{tabular}                                      &              &              & 0.077                                                                                 &                                                                                 &                                                                                                    \\ 
\hline
\begin{tabular}[c]{@{}l@{}}MLE Forecaster \\+ Planner (0.25s)\\(Class B)\end{tabular}               &              &              & 0.075                                                                                 &                                                                                 &                                                                                                    \\ 
\hline
\begin{tabular}[c]{@{}l@{}}MLE Forecaster \\+ Planner (1s)\\(Class B)\end{tabular}                  & 0.28         & 0.18         & 0.073                                                                                 & 0.91\%                                                                          & 0.18\%                                                                                             \\ 
\hline
\begin{tabular}[c]{@{}l@{}}MLE Forecaster \\+ Planner \\w col loss (1s)\\(Class B)\end{tabular}     & 0.28         & 0.18         & 0.074                                                                                 & 0.69\%                                                                          & 0.14\%                                                                                             \\ 
\hline
\begin{tabular}[c]{@{}l@{}}MLE Forecaster \\+ Planner \\w min-max loss (1s)\\(Class C)\end{tabular} & 0.29         & 0.18         & 0.075                                                                                 & 0.76\%                                                                          & 0.16\%                                                                                            
\end{tabular}
\end{table}

==> inputs/tables/crowdnav_onpolicy.tex <==
\begin{table}
\label{tab:crowdnav_on}
\caption{On-Policy Evaluation on CrowdNav environment}
\centering
\begin{tabular}{l|l|l|l}
\textbf{Method}                                                                                     & \begin{tabular}[c]{@{}l@{}}\textbf{Suc. }\\\textbf{Rate}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Col.}\\\textbf{Rate}\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Reward~}\\\textbf{(+ std. dev)}\end{tabular}  \\ 
\hline
\begin{tabular}[c]{@{}l@{}}Vanilla IL \\(Class A)\end{tabular}                                      & 61\%                                                                  & 38\%                                                                 & 0.50 +- 0.61                                                                     \\ 
\hline
\begin{tabular}[c]{@{}l@{}}MLE Forecaster + \\Planner (0.25s)\\(Class B)\end{tabular}               & 65\%                                                                  & 34\%                                                                 & 0.50 +- 0.61                                                                     \\ 
\hline
\begin{tabular}[c]{@{}l@{}}MLE Forecaster + \\Planner (1s)\\(Class B)\end{tabular}                  & 80\%                                                                  & 20\%                                                                 & 0.74 +- 0.50                                                                     \\ 
\hline
\begin{tabular}[c]{@{}l@{}}MLE Forecaster + \\Planner w \\col loss (1s)\\(Class B)\end{tabular}     & 73\%                                                                  & 26\%                                                                 & 0.66 +- 0.55                                                                     \\ 
\hline
\begin{tabular}[c]{@{}l@{}}MLE Forecaster + \\Planner w \\min-max loss (1s)\\(Class C)\end{tabular} & 78\%                                                                  & 22\%                                                                 & 0.71 +- 0.52                                                                    
\end{tabular}
\end{table}
